Answer ranking in Community Question Answering: a deep learning approach

Community Question Answering is the field of computational linguistics that deals with problems derived from the questions and answers posted to websites such as Quora or Stack Overflow. Among some of these problems we find the issue of ranking the multiple answers posted in reply to each question by how informative they are in the attempt to solve the original question. This work tries to advance the state of the art on answer ranking for community Question Answering by proceeding with a deep learning approach. We started off by creating a large data set of questions and answers posted to the Stack Overflow website. We then leveraged the natural language processing capabilities of dense embeddings and LSTM networks to produce a prediction for the accepted answer attribute, and present the answers in a ranked form ordered by how likely they are to be marked as accepted by the question asker. We also produced a set of numerical features to assist with the answer ranking task. These numerical features were either extracted from metadata found in the Stack Overflow posts or derived from the questions and answers texts. We compared the performance of our deep learning models against a set of forest and boosted trees ensemble methods and found that our models could not improve the best baseline results. We speculate that this lack of performance improvement versus the baseline models may be caused by the large number of out of vocabulary words present in the programming code snippets found in the questions and answers text. We conclude that while a deep learning approach may be helpful in answer ranking problems new methods should be developed to assist with the large number of out of vocabulary words present in the programming code snippets

==> _evaluation.tex <==
\chapter{Evaluation}

TODO add intro, explain better

As we have seen when the data set was described the original class distribution for the accepted answer feature is very unbalanced, hence using a classical binary classification metric such as accuracy would be misleading since a naive model that predicted all answers to not be accepted would yield a large accuracy values.

Due to this class unbalancing it was decided to use figures of merit from the information retrieval field, where multiple results are available for a single query and different metrics allow to easily compare between the different results which ones have been better classified or ranked. The information retrieval metrics we will use are the Mean Reciprocal Rank (MRR) \cite{voorhees-tice-2000-trec} and the Normalized Discounted Cumulative Gain (NDCG) \cite{10.1145/582415.582418}. 

It was decided to discard the usage of Mean Average Precision (MAP) metric which is the most common in information retrieval problems

Indicar que descartas Mean Average Precision (MAP), que es la medida más común en IR, porque sólo tienes una respuesta correcta por pregunta y en ese caso MAP es igual a MRR.

In order to define the Mean Reciprocal Rank we will first define the Reciprocal Rank. The Reciprocal Rank measure calculates the reciprocal of the rank at which the first relevant document resulting from an information retrieval query was retrieved. In our case this first relevant document will be the answer accepted by the user who asked the question. Given that we will be evaluating our experiments over a collection of questions and answers sets we will compute the average Reciprocal Rank over all the questions and corresponding answers sets, hence yielding the Mean Reciprocal Rank figure.

\[RR = \sum_{i=1}^{M} \frac{1}{rank_i} \]
\captionof{figure}{Reciprocal Rank equation}

\[MRR = \frac{1}{N} \sum_{i=1}^{N} RR_i \]
\captionof{figure}{Mean Reciprocal Rank equation}

The Normalized Discounted Cumulative Gain is another metric from the information retrieval field that measures the performance of an information retrieval system (most frequently a search engine) by ranking the results according to the their relevance in terms of the search query. In order to compute the Normalized Discounted Cumulative Gain we first must calculate the 
Discounted Cumulative Gain (DCG), this is the sum of the relevance scores of each of the query results divided by a discount factor such that lower ranking results have a smaller effect on the cumulative gain sum.

\[DCG_k = \sum_{i=1}^{k} \frac{relevance_i}{log_2 (i+1)} \]
\captionof{figure}{Discounted Cumulative Gain equation}

Then we will compute the Normalized Discounted Cumulative Gain by dividing the Discounted Cumulative Gain by the Ideal Discounted Cumulative Gain (IDCG), this is the DCG value for a perfect query, where each of the results has the actual importance.

\[NDCG_k = \frac{DCG_k}{IDCG_k}\]
\captionof{figure}{Normalized Discounted Cumulative Gain equation}

In the specific case of our experiments we will consider that the ideal relevance scores will take the form of a unity value for the accepted answer and zero for the rest of the answers.

We will see some examples of how these metrics will allow us to measure how well our models perform. Let us consider two arrays of values, one corresponding to the ground truth for the accepted answer and one for the model output. For the ground truth the array will resemble a one hot encoded vector, where only the index relative to the accepted answer is set to one will the other elements are set to zero. On the other hand the array corresponding to the model output will contain a graduation of values belonging to the probability that each of the answers to a question is the accepted answer, as predicted by the model under evaluation.

We will first consider the case of a perfect prediction, where the correct answer was perfectly identified. Hence we will have 2 arrays of data, the first one $r_{gold}$ that contains the ground truth of the accepted answer and $r_{eval}$ with the model output. In the case of a perfect input the value of each array will be

\[r_{gold}=\{0,0,1\}\ \, r_{eval}=\{0,0,1\}\]

On this example MRR and NDCG respectively will be 1.0 and 1.0 for this input.

We will now consider the case for the worst case prediction error. In this case $r_{gold}$ again contains the ground truth of the accepted answer and $r_{eval}$ with the model output, where the accepted answer was not the correct one:

\[r_{gold}=\{0,0,1\}\ \, r_{eval}=\{0,1,0\}\]

In this case MRR and NDCG respectively will be 0.333 and 0.565.
